Goal-driven text descriptions for images

A big part of achieving Artificial General Intelligence(AGI) is to build a machine that can see and listen like humans. Much work has focused on designing models for image classification, video classification, object detection, pose estimation, speech recognition, etc., and has achieved significant progress in recent years thanks to deep learning. However, understanding the world is not enough. An AI agent also needs to know how to talk, especially how to communicate with a human. While perception (vision, for example) is more common across animal species, the use of complicated language is unique to humans and is one of the most important aspects of intelligence. In this thesis, we focus on generating textual output given visual input. In Chapter 3, we focus on generating the referring expression, a text description for an object in the image so that a receiver can infer which object is being described. We use a comprehension machine to directly guide the generated referring expressions to be more discriminative. In Chapter 4, we introduce a method that encourages discriminability in image caption generation. We show that more discriminative captioning models generate more descriptive captions. In Chapter 5, we study how training objectives and sampling methods affect the models' ability to generate diverse captions. We find that a popular captioning training strategy will be detrimental to the diversity of generated captions. In Chapter 6, we propose a model that can control the length of generated captions. By changing the desired length, one can influence the style and descriptiveness of the captions. Finally, in Chapter 7, we rank/generate informative image tags according to their information utility. The proposed method better matches what humans think are the most important tags for the images.

==> colorcode.tex <==
\begin{figure*}[!h]
  \centering
\begin{tikzpicture}[every node/.style={font=\footnotesize}]
  \definecolor{aeroplane-co}{rgb}{0.502,0,0}
    \node[text=white,fill=aeroplane-co,draw=aeroplane-co,minimum
    height=0.6cm,minimum width=0.9cm] (aeroplane) {aeroplane};

    \definecolor{bicycle-co}{rgb}{0,0.502,0}    
    \node[text=white,fill=bicycle-co,draw=bicycle-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of aeroplane,right=.1cm] (bicycle) {bicycle};

    \definecolor{bird-co}{rgb}{0.502,0.502,0}    
    \node[text=white,fill=bird-co,draw=bird-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of bicycle,right=.1cm] (bird) {bird};

    \definecolor{boat-co}{rgb}{0,0,0.502}    
        \node[text=white,fill=boat-co,draw=boat-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of bird,right=.1cm] (boat) {boat};

    \definecolor{bottle-co}{rgb}{0.502,0,0.502}    
    \node[text=white,fill=bottle-co,draw=bottle-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of boat,right=.1cm] (bottle) {bottle};
    
    \definecolor{bus-co}{rgb}{0,0.502,0.502}    
    \node[text=white,fill=bus-co,draw=bus-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of bottle,right=.1cm] (bus) {bus};

    \definecolor{car-co}{rgb}{0.502,0.502,0.502}    
    \node[text=white,fill=car-co,draw=car-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of bus,right=.1cm] (car)
    {car};

    \definecolor{cat-co}{rgb}{0.251,0,0}    
    \node[text=white,fill=cat-co,draw=cat-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of car,right=.1cm] (cat)
    {cat};

    \definecolor{chair-co}{rgb}{0.753,0,0}    
    \node[text=white,fill=chair-co,draw=chair-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of cat,right=.1cm] (chair)
    {chair};

    \definecolor{cow-co}{rgb}{0.251,0.502,0}    
    \node[text=white,fill=cow-co,draw=cow-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of chair,right=.1cm] (cow)
    {cow};

	\definecolor{diningtable-co}{rgb}{0.753,0.502,0}    
    \node[text=white,fill=diningtable-co,draw=diningtable-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of cow,right=.1cm] (diningtable)
    {diningtable};


%    \definecolor{diningtable-co}{rgb}{0.753,0.502,0}    
%    \node[text=white,fill=diningtable-co,draw=diningtable-co,minimum
%    height=0.6cm,minimum width=0.9cm,below=of aeroplane,below=.1cm] (diningtable)
%    {diningtable};

    \definecolor{dog-co}{rgb}{0.251,0,0.502}    
    \node[text=white,fill=dog-co,draw=dog-co,minimum
    height=0.6cm,minimum width=0.9cm,below=of aeroplane,below=.1cm] (dog)
    {dog};

    \definecolor{horse-co}{rgb}{0.753,0,0.502}    
    \node[text=white,fill=horse-co,draw=horse-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of dog,right=.1cm] (horse)
    {horse};

    \definecolor{motorbike-co}{rgb}{0.251,0.502,0.502}    
    \node[text=white,fill=motorbike-co,draw=motorbike-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of horse,right=.1cm] (motorbike)
    {motorbike};

    \definecolor{person-co}{rgb}{0.753,0.502,0.502}    
    \node[text=white,fill=person-co,draw=person-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of motorbike,right=.1cm] (person)
    {person};

    \definecolor{pottedplant-co}{rgb}{0,0.251,0}    
    \node[text=white,fill=pottedplant-co,draw=pottedplant-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of person,right=.1cm] (pottedplant)
    {pottedplant};

    \definecolor{sheep-co}{rgb}{0.502,0.251,0}    
    \node[text=white,fill=sheep-co,draw=sheep-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of pottedplant,right=.1cm] (sheep)
    {sheep};

    \definecolor{sofa-co}{rgb}{0,0.753,0}    
    \node[text=white,fill=sofa-co,draw=sofa-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of sheep,right=.1cm] (sofa)
    {sofa};

    \definecolor{train-co}{rgb}{0.502,0.753,0}    
    \node[text=white,fill=train-co,draw=train-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of sofa,right=.1cm] (train)
    {train};

   \definecolor{tvmonitor-co}{rgb}{0,0.251,0.502}    
    \node[text=white,fill=tvmonitor-co,draw=tvmonitor-co,minimum
    height=0.6cm,minimum width=0.9cm,right=of train,right=.1cm] (tvmonitor)
    {tvmonitor};


\end{tikzpicture}
  \caption{Color code for VOC categories. Background is black.}
  \label{fig:colorcode}
\end{figure*}


==> copyright.tex <==

% \clearpage


% \vspace*{\fill}

% Copyright \textcopyright\ (Ruotian Luo) All rights reserved.

% \clearpage

% from https://www.mccormick.northwestern.edu/applied-math/documents/general/nuthesis.cls
\def\copyrightpage{%
  \clearpage
\begin{center}
  \ \\
  \vspace{\fill}
\copyright \ Copyright by \thesisAuthor \ 2021 \\
All Rights Reserved
\vspace{\fill}
\end{center}}
\def\endcopyrightpage{\newpage}

\copyrightpage

==> mainfig.tex <==
\begin{figure}[!th]
\centering
  \begin{tikzpicture}
% boundary pixels for regions saved by msk2txt
% coordinates of N3 obtained by:
% 1) Ns=neighborhoodSet(neighbors,3,252);
% 2) msk=false(size(suppix)); for n=1:length(Ns), msk=msk|suppix==Ns(n); end
% 3) pix2tikz([],[],msk,size(im,2)/7)
%   where 7 = width in cm (minimum width value in \node)
    \node[rectangle,draw=black,thick,fill overzoom
    image=figs/2007_003143.jpg,minimum width=7cm,minimum height=4.08cm,opacity=.5] (image) {};
    \node[fit=(image),draw=green!60!black,line width=2pt,inner
    sep=0pt,opacity=.8] (global) {};
    
    % superpixel
    \draw[red,line width=1pt] plot[smooth] file {figs/2007_003143_suppix252.txt};
    % levels
    \draw[name path=zo2,cyan,line width=1pt] plot[smooth] file {figs/2007_003143_sp252_zo1.txt};

    \draw[name path=zo6,olive,line width=1pt] plot[smooth] file {figs/2007_003143_sp252_zo6.txt};

    \draw[name path=zo10,blue!50!red,line width=1pt] plot[smooth] file {figs/2007_003143_sp252_zo10.txt};

    \draw[name path=zo13,blue!80!black,line width=1pt] plot[smooth] file {figs/2007_003143_sp252_zo13.txt};

    % N3
    \node[rectangle,draw=orange,line width=2pt,minimum
    width=2.492cm,minimum height=1.904cm,opacity=.8] (n3) at (-1.295,-0.189) {};
    
    % feature vector
    \node[above=of global.north west,above=15pt] (flocal) {\textcolor{cyan}{$\bfgreek{phi}_1$}};
    \node[right=of flocal,right=0pt] (dots1) {\ldots};
    \node[right=of dots1,right=0pt] (f6) {\textcolor{olive}{$\bfgreek{phi}_6$}};
    \node[right=of f6,right=0pt] (dots2) {\ldots};
    \node[right=of dots2,right=0pt] (f10) {\textcolor{blue!50!red}{$\bfgreek{phi}_{10}$}};
    \node[right=of f10,right=0pt] (dots3) {\ldots};
    \node[right=of dots3,right=0pt] (f13) {\textcolor{blue!80!black}{$\bfgreek{phi}_{13}$}};
    \node[right=of f13,right=0pt] (fn3) {\textcolor{orange}{$\bfgreek{phi}_{window}$}}; 
    \node[right=of fn3,right=0pt] (fglobal) {\textcolor{green!60!black}{$\bfgreek{phi}_{scene}$}}; 
    \node[fit=(flocal)(fglobal),inner sep=0pt,draw=black,thick]
    (feat) {};

    % arrows (manual; need to figure out how to automate)
    \coordinate (pt1) at (-1.456,0);
    \draw[thick,cyan,-latex] (pt1) -- (flocal);

    \coordinate (pt6) at (-1.218,0.210);
    \draw[thick,olive,-latex] (pt6) -- (f6);

    \coordinate (pt10) at (0.224,0.700);
    \draw[thick,blue!50!red,-latex] (pt10) -- (f10);

    \coordinate (pt13) at (0.644,1.498);
    \draw[thick,blue,-latex] (pt13) -- (f13);

    \coordinate (ptw) at (0.042,-0.140);
    \draw[thick,orange,-latex] (ptw) -- (fn3);

    \path (image.north east) -- ++(-.5,0) coordinate (ptglobal);
    \draw[thick,green!60!black,-latex] (ptglobal) -- (fglobal);

    \node[above=of feat,draw=black,thick,above=10pt] (mlp)
    {multi-layer perceptron};
    \draw[thick,-latex] (feat)--(mlp);
    \draw[thick,-latex] (mlp.north) -- ++(0,10pt) node[above] {``car''};
  \end{tikzpicture}
  \caption{Schematic description of our approach. Features are
    extracted from a nested sequence of ``zoom-out'' regions around
    the superpixel at hand (red). Here we show four out of
    thirteen levels: 1
    (cyan), 6 (olive), 10 (purple) and 13 (blue), as well as the
    window level (orange) and scene level (green). The features
    computed at all levels are comcantenated and fed to a multi-layer
    perceptron that classifies the superpixel.}\label{fig:main}
\end{figure}


==> notation.tex <==
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\mathA}{\mathbb{A}}
\newcommand{\mathB}{\mathbb{B}}
\newcommand{\mathC}{\mathbb{C}}
\newcommand{\mathD}{\mathbb{D}}
\newcommand{\mathE}{\mathbb{E}}
\newcommand{\mathF}{\mathbb{F}}
\newcommand{\mathG}{\mathbb{G}}
\newcommand{\mathH}{\mathbb{H}}
\newcommand{\mathI}{\mathbb{I}}
\newcommand{\mathJ}{\mathbb{J}}
\newcommand{\mathK}{\mathbb{K}}
\newcommand{\mathL}{\mathbb{L}}
\newcommand{\mathM}{\mathbb{M}}
\newcommand{\mathN}{\mathbb{N}}
\newcommand{\mathO}{\mathbb{O}}
\newcommand{\mathP}{\mathbb{P}}
\newcommand{\mathQ}{\mathbb{Q}}
\newcommand{\mathR}{\mathbb{R}}
\newcommand{\mathS}{\mathbb{S}}
\newcommand{\mathT}{\mathbb{T}}
\newcommand{\mathU}{\mathbb{U}}
\newcommand{\mathV}{\mathbb{V}}
\newcommand{\mathW}{\mathbb{W}}
\newcommand{\mathX}{\mathbb{X}}
\newcommand{\mathY}{\mathbb{Y}}
\newcommand{\mathZ}{\mathbb{Z}}

\newcommand{\vecA}{\mathbf{A}}
\newcommand{\vecB}{\mathbf{B}}
\newcommand{\vecC}{\mathbf{C}}
\newcommand{\vecD}{\mathbf{D}}
\newcommand{\vecE}{\mathbf{E}}
\newcommand{\vecF}{\mathbf{F}}
\newcommand{\vecG}{\mathbf{G}}
\newcommand{\vecH}{\mathbf{H}}
\newcommand{\vecI}{\mathbf{I}}
\newcommand{\vecJ}{\mathbf{J}}
\newcommand{\vecK}{\mathbf{K}}
\newcommand{\vecL}{\mathbf{L}}
\newcommand{\vecM}{\mathbf{M}}
\newcommand{\vecN}{\mathbf{N}}
\newcommand{\vecO}{\mathbf{O}}
\newcommand{\vecP}{\mathbf{P}}
\newcommand{\vecQ}{\mathbf{Q}}
\newcommand{\vecR}{\mathbf{R}}
\newcommand{\vecS}{\mathbf{S}}
\newcommand{\vecT}{\mathbf{T}}
\newcommand{\vecU}{\mathbf{U}}
\newcommand{\vecV}{\mathbf{V}}
\newcommand{\vecW}{\mathbf{W}}
\newcommand{\vecX}{\mathbf{X}}
\newcommand{\vecY}{\mathbf{Y}}
\newcommand{\vecZ}{\mathbf{Z}}
\newcommand{\vecAlpha}{\boldsymbol{\alpha}}
\newcommand{\vecBeta}{\boldsymbol{\beta}}
\newcommand{\vecGamma}{\boldsymbol{\gamma}}
\newcommand{\vecLambda}{\boldsymbol{\lambda}}
\newcommand{\vecDelta}{\boldsymbol{\Delta}}
\newcommand{\vecdelta}{\boldsymbol{\delta}}
\newcommand{\vecphi}{\boldsymbol{\phi}}
\newcommand{\vectheta}{\boldsymbol{\theta}}

\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vech}{\mathbf{h}}
\newcommand{\veci}{\mathbf{i}}
\newcommand{\vecj}{\mathbf{j}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\vecl}{\mathbf{l}}
\newcommand{\vecm}{\mathbf{m}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\veco}{\mathbf{o}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\vecs}{\mathbf{s}}
\newcommand{\vect}{\mathbf{t}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecz}{\mathbf{z}}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\length}{len}

\newcommand{\removed}[1]{}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\one}[1]{\left[\!\left[ #1 \right]\!\right]}
\newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin}} \:}
\newcommand{\argmax}[1]{\underset{#1}{\mathrm{argmax}} \:}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\E}[1]{{\mathbb{E}\left[{#1}\right]}}
\newcommand{\hE}[1]{{\mathbb{\hat{E}}\left[{#1}\right]}}
\newcommand{\Ep}[2]{{\mathbb{E}_{#1}\left[{#2}\right]}}
\newcommand{\hinge}[1]{[#1]_+}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\abs}[1]{{\left\lvert{#1}\right\rvert}}
\newcommand{\margin}{\text{margin}}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\pr}[2]{{\mathbb{P}_{#1}\left[{#2}\right]}}

\newcommand{\net}{\text{net}}
\newcommand{\eps}{\epsilon}
\newcommand{\tW}{\widetilde{W}}
\newcommand{\In}{\text{in}}
\newcommand{\Out}{\text{out}}
\newcommand{\Win}{\vecW_{\text{in}}}
\newcommand{\Wout}{\vecW_{\text{out}}}
\newcommand{\Wrec}{\vecW_{\text{rec}}}
\newcommand{\relu}{\sigma_{\textsc{relu}}}
\newcommand{\err}{Err}
\newcommand{\error}{\epsilon}
\newcommand{\hatD}{\widehat{D}}
\newcommand{\hatL}{\hat{L}}
\newcommand{\hatl}{\hat{\ell}}

\newcommand{\vin}{v_{\textrm{in}}}
\newcommand{\vout}{v_{\textrm{out}}}
\newcommand{\layer}{\text{layer}}
\newcommand{\gnorm}[1]{\norm{#1}}
\newcommand{\pathr}{\phi}
\newcommand{\DAG}{\text{DAG}}
\newcommand{\convexnn}{\nu}
\newcommand{\nout}{n_\text{out}}
\newcommand{\nin}{n_\text{in}}
\newcommand{\netdepth}{d}
\newcommand{\netwidth}{H}
\newcommand{\nparam}{n_{\text{param}}}

==> sections/moe_captioning.tex <==
\chapter{Mixture of Experts based diverse captioning}\label{chap:ref_exp}




==> sections/tagging/scratch.tex <==

% =========
FROM INTRO 
% =========

% Tag2Cap model generates a set of tags that optimize caption reconstruction. R means random sample a subset from the tags of image i. The sets that reconstruct the caption best is later used as ground truth for the generation model.




%% background
%We are interested in image tagging. The traditional automatic classifier can produce a large number of labels but often not-interesting.(\rtcom{Copy from IOTA}). Specifically, we want to generate a sequence of tags for an image ranked by their informativeness. \rtcom{Some figure 1 to illustrate the idea}
%
%% background on IOTA
%Previous work IOTA has considered injecting the notion of informativeness, which is measured by how the produced tag can reduce the uncertainty of the mental picture of the described image (speaker-listener).

% our motivation
%However, IOTA treats every category the same (\rtcom{not very correct}). A tag can be semantically important (a tag can induce many other related tags, e.g., dining table -> dishes, cups), but not be visually important/salient in the image (the dining table at the corner of an image). 

%Ideally, we would like only to say the most salient/informative things so that it can give the best idea of what the image is about \ake{we would like this in a captioning system? it sounds like you might be talking about humans with this wording, and I don't think that's what you mean}. We will denote this property of saliency/informativeness as ``utility''. Following this intuition \ake{that captioning systems should maximize utility of their outputs}, we propose a different \ake{different from what?} way that considers the utility of the tags in describing the image. We define utility as

%\begin{equation}
%    \mathcal{U}(w) = xxx
%\end{equation}\label{eq:utility}

%\lior{maybe add here [ formal definition of information utility (+refs)]. We measure utility in practice by caption reconstruction objective and define it as [equation tag utility].  (*) stronger justfication for why caption reconstruction reflects utility (the gloss intuition)}

% IOTA: tree structure is limited (biased to labels that are hubs); only one label; not considering utility.

% brief our method

%The idea of selecting tags based on criteria of usefulness and information content is also not new~\cite{grice1975logic,wilson2002relevance}. Unfortunately, these concepts are very difficult to quantify and measure in practice. In this paper we consider concrete definitions for information utility as defined above, yielding computational models for maximizing utility in generating image tags.  %\ake{where has this been argued? do you mean that it has been argued that people likely \emph{will} select tags based on these criteria? (and if so, still refer back to first question :-) ) Maybe you intend to refer to more general principles of how people choose to convey information.}.\gs{need refs!}\gal{Added refs}  
%\gs{attempt at clarification} \ake{yeah this is clearer. I made slight tweaks and added comments}

%\gs{??}\ake{okay I think this is starting to explain the reason for using tags---might want to give that justification above where people are likely to wonder immediately about why we use tags}


%To evaluate the usefulness of tags, we leverage on the fact that images are often described with captions, and large datasets of image captions have been collected \cite{lin2014microsoft,sharma-etal-2018-conceptual}. We use such captions to quantify the utility of how well the tags can describe the image, by training  a tag to caption (\tagcap) model which can reconstruct a full caption from a set of keywords/tags. With this \tagcap model we can measure how well each possible tag can reconstruct the captions of a particular image, and treat that as the informativeness/utility (assuming we have a set of golden captions as reference).% The reason why we want to reconstruct the captions because captions are how humans describe an image. 

 %The tag2cap model is similar to the chow-liu tree model in IOTA in representing a world model of the listener; the difference is, instead of measuring uncertainty, we measure how well it can reconstruct the image content.

%\gal{The following is not clear} \ake{agree things get a little confusing here} Similarly, in addition to captions, we also attempt to measure the informativeness by looking at how good the tags are at reconstructing the image features/image tags which are alternative representations of the image content. We found \tagcap wins because it captures the utility.
% tag2cap
% why tagging?
% Gal: We dont really need the following now
%While it looks over-killed to generate tags when having captions, there has been recent work that treats generating tags as an intermediate step for generating better captions. Our work can be treated as a better variant to generate tags.

% our test settings
% \ake{The below level of detail about the evaluation probably not needed in the introduction. I think the key thing for the intro will be to ground the motivation in information utility, and then introduce and justify this sequential tagging scheme as a way of looking at information utility. (This is what you've gotten started doing above)} We study two  settings of the tag-evaluation  task. First, \textbf{\textit{tag-ranking}}, where the tags are given, and the goal is to rank them in the order of informativeness; for simplicity these tags are all correct tags for the image. To rank the tags we can use additional information other than raw pixels, like image features, captions and tags, for reference. 


% % test set
% \gal{Move from the intro to later section}
% For evaluation, we collect a test set of 1k images. For each image, we ask 10 turkers to say the most important thing, free-formly. After extracting the first most important tag, we ask the turkers to emit the second important thing in addition to the first tag. We do this for three rounds, and are able to get a tag sequence ordered by importance. We compare the results of human and the output of the models to look at the performance. See Table \ref{table:eval}.


% \lior{General comments: (1) since its ACL we might want to emph that vision side; that will separate us from a lot of other papers in the field. (2) In the methods section i think it would be helpful to give a best and worst case example.}

% =====================
FROM RELATED WORK
% =====================
% % from Orderless related work.
% Earlier works that tried to leverage label correlations
% exploited graphical models such as Conditional Random
% Fields (CRFs) [. Collective multilabel classification] or Dependency Networks [Multi-label classification using conditional dependency networks]. Chen
% et al. [Learning deep structured models] combine CRFs with deep learning algorithms to
% explore dependencies between the output variables. Read
% et al. [Classifier chains for multi-label classification] propose using a chain of binary classifiers to
% do multi-label classification. Most of the approaches mentioned come with relatively high computation costs since
% they need to model explicitly the pairwise label correlation

% % from elucidating
%  In order to explicitly exploit
% label co-occurrences, researchers have resorted to modeling the joint probability distribution of labels [59] or decomposing the joint distribution into conditionals [11, 61,
% 45, 28, 32, 41, 46].

% Alternative solutions to capture label co-occurrences
% include learning joint input-label embeddings with rankingbased losses [66, Multi-label classification via feature-aware implicit label
% space encoding, Learning deep latent spaces for multilabel classification,  Improving pairwise
% ranking for multi-label image classification, Deep convolutional ranking for multilabel image annotation], graph neural networks
% [Multi-label image recognition with graph convolutional networks], and using loss functions that directly account for those
% [15, 63, 42, 54]. 


% \cite{leong2010text} - Text Mining for Automatic Image Tagging
% \cite{li2011composing} - Composing Simple Image Descriptions using Web-scale N-grams; , Tamara L Berg, Alexander C Berg, and Yejin Choi; 2011; 20 citations
% \cite{tariq2016context} - A Context-Driven Extractive Framework for Generating Realistic Image Descriptions

% \cite{tan2020progressive} propose a method for generating long text by first producing content keywords and then progressively refining them into complete passages in multiple
% stages.

% coarse to fine generation: from SOE intro

% Tan et al. (2020) takes a multi-step strategy, which progressively refines the generated incomplete text until reaching a specified stage

% https://arxiv.org/pdf/2010.07074.pdf - Summarize, Outline, and Elaborate
% \lior{This was published in ArXiv2020 - very similar to ours; tried to formulate how our work is different. RT - is this accurate?} \rtcom{It is very similar in idea after a glance.}
% Similar to the idea of generating text based on gloss, \cite{sun2020summarize} propose SOE, a model that generates the most informative words to reconstruct a text segment. 

% They are focused in a coarse-to-fine parsing where we consider more complex tag interdependencies.

%%%% LB - I'm commenting out this section; we have it twice + Comments implemented. %%%% 
% % compare to tan et al. move from methods
% This is similar to \cite{tan2020progressive}. The difference is, in our setting, the input is an unordered set of tags, where in \cite{tan2020progressive}, the input is a sequence of words. \ake{This is something good to include in related work, but it's not inappropriate to mention here as well. More importantly, say why we do it differently}

%%%%%%%%%%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% 

% Check: 
% 1. https://www.aclweb.org/anthology/2020.acl-main.586.pdf ;  Words Aren’t Enough, Their Order Matters ; ACL20 ; FAIR
% 2. Annotation Order Matters: Recurrent Image Annotator for Arbitrary Length Image Tagging https://arxiv.org/pdf/1604.05225v3.pdf 2016 % added
% 3. From Greg: Evaluating the Factual Consistency of Abstractive Text Summarization; Socher 2019 - factual consistency. We can ague that vision grounding helps that 
% 4. Multi-Image Summarization: Textual Summary from a Set of Coherent Images



% =================
FROM EXP
% =================

% \begin{table*}[htbp]
% \begin{minipage}[c]{.215\textwidth}
%     \includegraphics[height=1in]{figs/000000091045.jpeg}
%     \caption{\small Evaluations set. In three rounds people are asked what is the important in the image. Each round we condition on a label set (in red).}\label{table:rounds}
% \end{minipage}
% \hfill % minipage justification (creates the space between the two.
% \begin{minipage}[c]{120mm}
% \begin{center}
%     % \small
%     \scalebox{0.84}{ 
%         \begin{tabular}{l|ll|ll}
%         \textbf{Round 1} & \multicolumn{2}{c}{\textbf{Round 2}} & \multicolumn{2}{c}{\textbf{Round 3}} \\\hline
%  & \textit{\textbf{\textcolor{red}{people}}} & \textit{\textbf{\textcolor{red}{men}}} & \textit{\textbf{ \textcolor{red}{people, men}}}     & \textit{\textbf{ \textcolor{red}{people, party} }}     \\ \hline
%         Smiling &  men  & cocktails in a museum    & wine  & suits    \\
%         people  &  men    & party  &   artwork &  artwork  \\
%         Friends &  party     &   suits     &  party guests & tie \\
%         People  &  party &    woman       &     Suit & Painting \\
%         wedding reception   & celebrating  & smiling  & picture  & glass \\
%         two men  & Friends  & cheers & artwork & Drink\\
%         men in suits & two &  tuxedo     &  Drink  & painting\\
%         Men in suites      &humans      & suits & Suits & drinks \\
%         drunk friends & men & drinking      &art  & men  \\
%         people  &    drinks    & smile &tie & Men
%         \end{tabular}
%     }
% \end{center}
% \end{minipage}
% \end{table*}


% \begin{table*}[htbp]
% \begin{minipage}[c]{.215\textwidth}
%     \includegraphics[height=0.9in]{figs/000000091045.jpeg}
%     \caption{\small Evaluations set. In three rounds people are asked what is the important in the image. Each round we condition on a label set (in red). \textit{Top row} is the raw answers from turkers; and \textit{bottom row} shows the set of tags after processing (lemmatization etc.) and the final label count}\label{tab:eval}
% \end{minipage}
% \hfill % minipage justification (creates the space between the two.
% \begin{minipage}[c]{120mm}
% \begin{center}
%     % \small
%     \scalebox{0.84}{ 
%         \begin{tabular}{l|ll|ll}
%         \textbf{Round 1} & \multicolumn{2}{c}{\textbf{Round 2}} & \multicolumn{2}{c}{\textbf{Round 3}} \\\hline
%  & \textit{\textbf{\textcolor{red}{people}}} & \textit{\textbf{\textcolor{red}{men}}} & \textit{\textbf{ \textcolor{red}{people, men}}}     & \textit{\textbf{ \textcolor{red}{people, party} }}     \\ \hline
%         Smiling &  men  & cocktails in a museum    & wine  & suits    \\
%         people  &  men    & party  &   artwork &  artwork  \\
%         Friends &  party     &   suits     &  party guests & tie \\
%         People  &  party &    woman       &     Suit & Painting \\
%         wedding reception   & celebrating  & smiling  & picture  & glass \\
%         two men  & Friends  & cheers & artwork & Drink\\
%         men in suits & two &  tuxedo     &  Drink  & painting\\
%         Men in suites      &humans      & suits & Suits & drinks \\
%         drunk friends & men & drinking      &art  & men  \\
%         people  &    drinks    & smile &tie & Men \\\hline
%   &  	 &  	 & 	 & \\
%         \textbf{3} people    & \textbf{4} man   & \textbf{2} suit       & \textbf{3} artwork  & \textbf{2} painting \\
%         \textbf{3} man      & \textbf{4} human  & \textbf{2} smile      & \textbf{3} art    & \textbf{2} man \\
%         \textbf{2} friend	& \textbf{2} party  & \textbf{1} cocktail   & \textbf{2} suit  & \textbf{2} drink \\
%         \textbf{2} suit    & \textbf{1} celebrate& \textbf{1} museum     & \textbf{1} wine   & \textbf{1} suit \\
%         \textbf{1} smile   &\textbf{1} friend	& \textbf{1} party  & \textbf{1} party      & \textbf{1} artwork \\
%         \textbf{1} wedding  & \textbf{1} drink    & \textbf{1} woman  & \textbf{1}  guest     & \textbf{1} tie \\
%         \textbf{1} reception &         & \textbf{1} cheer  & \textbf{1}  party guest   & \textbf{1} glass \\
%         \textbf{1} wedding reception & & \textbf{1} tuxedo & \textbf{1} picture \\
%         \textbf{1 }drunk &    & \textbf{1} drinking   & \textbf{1}drink  \\
%         &  	 &  	 & 	\textbf{1} tie   & \\
%         \end{tabular}
%     }
% \end{center}
% \end{minipage}
% \end{table*}


% \begin{table}[htbp]
%   \small
%   \setlength{\tabcolsep}{1pt}
%     \centering
%     \begin{tabular}{l|p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}|p{1.1cm}}
%    & \small{\tagcap CNN} &  \small{\tagcap CNN + GT} & \small{\tfidf} &  \small{t2 cbs 50 tfidf}& \small{\tf} & \small{freq.}\\ \hline
%    \multirow{5}{*}{\includegraphics[height=0.4in]{figs/000000088485.jpg}} 
%    & & & frisbee & frisbee & frisbee &  man\\
%    & & & hand & man & woman & stand \\
%    & & & hold& yellow& hold & hold \\
%    & & & woman & hold& yellow &  person \\
%    & & & disc &white & smile &  young \\
%     \end{tabular}
%     \caption{Ranking by different methods. frequency-based ranking yields a correct but completely uninformative set. }
%     \label{table:examples2}%
% \end{table}


%  \lior{we need to find meaningful examples. showing different trends for dofferent methods if exist}

%==========================
FROM DATA COLLECTION
%==========================

%%%% DO NOT DELETE / MOVE THIS (LB)
% \begin{figure*}[ht]
% \begin{minipage}[c]{.215\textwidth}
%     \includegraphics[height=0.8in]{figs/coco/000000091045.jpeg}
%     \caption{\small Evaluations set. People are asked what is the most important thing in the image, in three rounds. Each round provides a set of labels (red) as context of what is already known. We do this for 2k images and collect 20 sets of tags per image. Here, ``people'' and ``men'' are the most frequent tags and thus pass as context to the next round}\label{table:rounds}
% \end{minipage}
% \hfill % minipage justification (creates the space between the two.
% \begin{minipage}[c]{120mm}
% \begin{center}
%     \scalebox{0.84}{ 
%         \begin{tabular}{l|ll|ll}
%         \textbf{Round 1} & \multicolumn{2}{c}{\textbf{Round 2}} & \multicolumn{2}{c}{\textbf{Round 3}} \\\hline
%           & \textit{\textbf{\textcolor{red}{people}}} & \textit{\textbf{\textcolor{red}{men}}} & \textit{\textbf{ \textcolor{red}{people, men}}}     & \textit{\textbf{ \textcolor{red}{people, party} }}     \\ \hline
%         Smiling &  men  & cocktails in a museum    & wine  & suits    \\
%         \textbf{people}  &  men    & party  &   artwork &  artwork  \\
%         Friends &  party     &   suits     &  party guests & tie \\
%         \textbf{People}  &  party &    woman       &     Suit & Painting \\
%         wedding reception   & celebrating  & smiling  & picture  & glass \\
%         two \textbf{men}  & Friends  & cheers & artwork & Drink\\
%         \textbf{men} in suits & two &  tuxedo              &  Drink  & painting\\
%         \textbf{Men} in suites      &humans      & suits & Suits & drinks \\
%         drunk friends & men & drinking               &art  & men  \\
%         \textbf{people}  &    drinks    & smile &tie & Men
%         \end{tabular}
%     }
% \end{center}
% \end{minipage}
% \end{figure*}


% ==================== narrow table red chair cat 


% \begin{table}[ht]
%     \centering
%     \resizebox{.47\textwidth}{!}{%
%         \begin{tabular}{l|l|ll|ll}
%             &\textbf{Round 1} & \multicolumn{2}{c}{\textbf{Round 2}} & \multicolumn{2}{c}{\textbf{Round 3}} \\\hline
%             &  & \textit{\textbf{\textcolor{red}{cat}}} & \textit{\textbf{\textcolor{red}{chair}}} & \textit{\textbf{ \textcolor{red}{cat, chair}}}     & \textit{\textbf{ \textcolor{red}{cat, lazy} }}     \\ \hline
%             \multirow{10}{*}{\includegraphics[width=1in]{figs/coco/000000023731.jpeg}} & Cat &  chair  & Cat    & wheels  & chair    \\
%             & Cat  &  chair    & cat  &   Lazy &  chair  \\
%             & cat chair &  chair  &   cat   &  red & chair \\
%             & cat lounging in chair  &  chair &  cat     & table & chair \\
%             & Cat   & Chair  & cat  & wheel  & nap \\
%             & cat on a chair & cat & Sleeping stage & chair\\
%             & Cat & chair &  cat              &  sleep  & chair\\
%             & cat on chair      & chair      & cat & room & chair \\
%             & cat & Lazy & cat  & floor  & chair  \\
%             & Cat sleeping & rolling    & cat & Table & chair
%         \end{tabular}
%         }
%      \caption{People are asked what is the most important thing in the image, in three rounds. Each round provides a set of labels (red) as context of what is already known. We do this for 2k images and collect 20 sets  per image.}\label{table:rounds}
% \end{table}


% ============ wide table cat on red chair ========================
% \begin{figure*}[ht]
% \begin{minipage}[c]{.215\textwidth}
%     \caption{\small People are asked what is the most important thing in the image, in three rounds. Each round provides a set of labels (red) as context of what is already known. We do this for 2k images and collect 20 sets  per image.}\label{table:rounds}
% \end{minipage}
% \hfill % minipage justification (creates the space between the two.
% \begin{minipage}[c]{120mm}
% \begin{center}
%     \scalebox{0.84}{ 
%         \begin{tabular}{l|l|ll|ll}
%             &\textbf{Round 1} & \multicolumn{2}{c}{\textbf{Round 2}} & \multicolumn{2}{c}{\textbf{Round 3}} \\\hline
%             &  & \textit{\textbf{\textcolor{red}{cat}}} & \textit{\textbf{\textcolor{red}{chair}}} & \textit{\textbf{ \textcolor{red}{cat, chair}}}     & \textit{\textbf{ \textcolor{red}{cat, lazy} }}     \\ \hline
%             \multirow{10}{*}{\includegraphics[width=1in]{figs/coco/000000023731.jpeg}} & Cat &  chair  & Cat    & wheels  & chair    \\
%             & Cat  &  chair    & cat  &   Lazy &  chair  \\
%             & cat chair &  chair  &   cat   &  red & chair \\
%             & cat lounging in chair  &  chair &  cat     & table & chair \\
%             & Cat   & Chair  & cat  & wheel  & nap \\
%             & cat on a chair & cat & Sleeping stage & chair & chair \\
%             & Cat & chair &  cat              &  sleep  & chair\\
%             & cat on chair      & chair      & cat & room & chair \\
%             & cat & Lazy & cat  & floor  & chair  \\
%             & Cat sleeping & rolling    & cat & Table & chair
%         \end{tabular}
%     }
% \end{center}
% \end{minipage}
% \end{figure*}


% ---------------------------
FROM DATA PROCESSING    
% ---------------------------
% We collected tags for a test set of 2k images, yielding a total of 60k annotations; 20 sequences per image of tags ordered by importance. \gal{$2000 \times 20 = ?$ } \lior{num_images 2000 x num_raters 10 x num_rounds but it doesn't belong here anyway}

% Repeating. Commenting out. 
% For each image, we asked 10 raters to tag the image with the most important tag in free-form fashion. After extracting the first most important tag, we asked raters to produce the second most important tag given the first tag.
% \rtcom{Repeating?}
% This was repeated for three rounds, 

% Following instructions:  Less than 1\% repeated \gal{WDYM?} \lior{see gregs comment at the end of the previous section}the given tag. 80\% of the raters described the image with one word, and less than 4\% used more than three words. 
% =====================
FROM METHODS
% =======================
% LIOR TODO: make the example in the text consisient in the figure. V
% Show just one caption in all the figures and in the text we sat that we can do it with 5 V
% Examples of sets of arbitrary length  3,4,5 V

% \gal{Lior, call me to discuss this figure}\lior{(1)revised by gals comments (2) RT, is that a good sketch of tag2cap architecture?} \rtcom{what is the two men in suits here?}\lior{Eq 1. remove it?} \rtcom{I guess the the confusion here is which one is the reference caption, two men in suits or two men stadning together .....}\lior{fixed, removig comm}




%====================================================
FROM EXP
%======================================================

\subsubsection{\textbf{\textit{Tag-ranking}}}
5 caption. Table \ref{tab:ranking_5cap}. Compared to other methods using 5 captions as reference, our \tagcap model performs the best at SetRecall@1 which means it can capture the most important tag better. When $k>=2$, TFIDF and TF performs close, and TF is better on the SetPrec@1.
(\rtcom{Why are we worse when k>2, some analysis????, but tf and tfidf is cheating right??? It's better if we have some better explanation. One reason could be: because the way we parsed the ground truth. If the first word is light, and the second is traffic (while the first should be traffic light?) Our method may suffer because given light, traffic is not that interesting. Another reason may be, the human would say things are relevant instead of exclusive to the given tags. As in Table 1.})

Compared to other baselines, \tagtag, \tagfeat, and IOTA, the models using captions for reference are generally better, indicating richfulness of captions.

(Caveat: althought \tagtag and \tagfeat and IOTA doesn't use 5 captions during test time, they do use 5 caption during training. (The tags are from 5 captions))

To improve \tagcap, we also try to combine it with other methods. When combined with \tagfeat, SetRecall@1 can further be imporved. Combining TF/TF-IDF with \tagcap can further improve over TF and TF-IDF even when k$\ge$2 where \tagcap is inferior to. However, that still performs worse on SetRecall@1 compared to \tagcap and \tagcap+\tagfeat. By combining \tagcap, \tagfeat and TF, we can achieve the best results on all metrics.

1caption Table \ref{tab:ranking_1cap}, the counting based method no longer works. TF-IDF is much worse than \tagcap and even a simple heuristic method \textsc{TagOrder}. Because the coco caption tends to start with the main object and then other details (e.g. a xxxx with yyyy ), \textsc{TagOrder} can perform reasonably well.
% \rtcom{IOTA not known yet}\lior{now known. resolve}
\tagcap outperforms all other baselines, when k$>$2 while \tagfeat performs the best when k = 1. When combing \tagcap with \tagfeat, the method can significantly improve over individual methods. % (except k=5, I don't know why).


\rtcom{Another try to summarize results}
Ranking 5caption:
Compare to baselines with captions as reference (TF, TF-IDF), our method significantly outperforms them on choosing the most important one. All methods that use captions as reference outperform baselines that do not, including \tagfeat which uses image feature.

To investigate how combinations of methods works, we combine \tagcap with \tagfeat/TF/TF-IDF/IOTA, and found that.

Although \tagfeat-only performs, combining \tagcap with \tagfeat can achieve better SetRecall@1 compared to \tagcap only. \tagcap combined with TF and TF-IDF can improve the performance on all metrics compared to TF/TF-IDF only, but drag down the score on SetRecall@1. We further combine \tagcap \tagfeat and TF, and found that leads to the best score on all entries.


Ranking 1 caption:
First, we also compare \tagcap with caption based methods TagOrder and TF-IDF. In this case we find a simple heuristic TagOrder is performs even better than TF-IDF, and \tagcap outperforms them which means \tagcap can better utilize the information in the caption. \tagcap is also better than \tagtag, Freq which does not use 

Besides, \tagfeat achieve the best SetRecall@1, while being worse when k$\ge$2 than \tagcap.

However, we found IOTA stands out in this situation, and perform better on than all methods when k$\ge$2, however with a low SetRecall@1.

When combining different methods, we found combining with \tagfeat always bring boost on SetRecall@k$\le$3. Combining IOTA and \tagcap leads to the best SetRecall@ k$\ge3$, because they both perform well when k is large, however, this leads to lowest SetRecall@1 among all combined methods. Combining with IOTA or \tagcap always improve. In the end, \tagcap + \tagfeat + IOTA leads to the best SetRecall@1,2, and \tagcap+IOTA leads to the best SetRecall@4,5 (Gaps between SetRecall@3 is close). 


(Note that the game changing in ranking with 1 cap is IOTA, without IOTA, the perform is much clearer, but IOTA kind of breaks the even.)



Generation 5 cap:
\tagcap perform better than other methods except TF, TF-IDF, while still the best for k=1.

Adding \tagfeat to \tagcap improves on all metrics over \tagcap.

Combining \tagcap with other method allways improves.

Overall, combining \tagcap with TF-IDF leads to the best SetRecall@1, while perform as good as combing with TF when k$\ge$2, and better than \tagcap + \tagfeat. Combining \tagcap \tagfeat and TF-IDF leads to the best genreation performance under 5 caption setting.


Generaiton 1cap:

\tagcap and \tagfeat outperforms baselines significantly on SetRecall@1 where \tagcap and \tagfeat are close.
When k$\ge$2 IOTA and PLA performs better.

Combing \tagcap and \tagfeat can improve over \tagcap or \tagfeat on all metrics. Combining with PLA always improve (However, not always outperform PLA itself).

Adding IOTA can slightly improve. (t2c+t2f+iota+pla vs. t2c+t2f+pla and t2c+t2f+iota vs t2c+t2f(slightly worse on k=1)).

The t2c+t2f+(iota)+pla performs the best when k$\le$3.


Overall conclusion:
The best method performed on SetRecall@1, always involves either tag2cap or tag2feat or the combination of both. In most of the cases, incorporating


Also ,we found gen 5cap worse then ranking 5cap and gneration 1cap is better than ranking 1cap.


% =====================
FROM METHOD 
% ==================================
% %This sequence of ranked tags is then used for training. 
% In our evaluation, we associate the generator trained by pseudo tags from a particular ranker with that ranker. Thus the ``\tagcap generator'' is the generator described above, trained with pseudo tags ranked by \tagcap.\gs{clear?}\rtcom{clear to me}\gal{I understand it, but a naive reader may not. I suggest instead: } During evaluation, the generator trained with tags ranked by the \tagcap ranker, is named ``''\tagcap generator'' (and similarly, for \tagfeat generator). \gal{end suggestions}.


%\textbf{Training and inference.} 
%\begin{align}
%    L = \sum_k P(\hat t_k|t_0, \hat t_{1\ldots k-1})
%\end{align}

% \gal{Not clear:} 

% For different models, the difference is the training objectives. Orderless uses the loss proposed in \cite{yazici2020orderless}, where there is no ground truth order specified. The model has to learn to generate the tags that maximize the tagging performance.

% For ordered model, we can specify different ground truth order for the model to learn. For example, for each sample, we can order the tags according to their tfidf so that we get a tag sequence. We ask the model to learn to generate that sequence just like a captioning model.

% \subsection{Tag2Cap for generation}
% \gal{This section should be strongly revised. Start with explaining the generation workflow and the architecture. The two subsections are very unclear. all terms should be defined. }

% no longer used
% \subsubsection{As loss}

% We first sample a tag sequence from $P_G$, denoted as ${\hat t}_{0\ldots n}$, and then we feed the tags to the Tag2Cap model, and compute the following.
% \begin{align}
%     L &= [\log P_{t2c}(c|\hat t_0) - \log P_{t2c}(c)] * P_G(\hat t_0) \nonumber\\
%         &+ [\log P_{t2c}(c|\hat t_0, \hat t_1) - \log P_{t2c}(c|\hat t_0)] * P_G(\hat t_1|\hat t_0) \nonumber\\
%         &+ [\log P_{t2c}(c|\hat t_0, \hat t_1,\hat t_2) - \log P_{t2c}(c|\hat t_0,\hat t_1)] * P_G(\hat t_2|t_0,\hat t_1) \nonumber \\
%         &\ldots
% \end{align}
% We derive this loss from REINFORCE algorithm, where we treat the log probability difference as reward.



%\gal{Give an overview of the approach and Describe the workflow. which components of the model are trained when, using which data etc.} \ake{this is also a good time to remind the reader of the overall goals (e.g., zeroing in on information utility), and how the methods you're about to describe relate to those goals}
% \lior{} We begin by training the \tagcap model with the objective of reconstructing a sentence based on some subset of words (Figure \ref{fig:tag2cap}). Following \eqref{eq:utility} this gives us a \textit{utility scores} by which we can now rank the tags. Then we use this sequence in two setups. The first is \lior{todo add ranking vs generation}


% ======================
FROM RESULTS 
% ======================

% We only evaluate on tag sequence for now.
% \subsubsection{Output format}
% \gal{Output of what?}
% Depending on the evaluation, we can have multiple ways of output format.

% \paragraph{Tag sequence evaluation}
% For evaluating the tag sequence generation, we output a sequence of tags, ordered by ``importance''. We evaluate by using metrics, set accuracy@k, k from 1 to 5.

% \paragraph{Single tag evaluation}
% For evaluating a single tag (the first tag, or the second tag given some first tag), the model gives each candidate tag a score; for this task, we can evaluate recall@k(k=1,2,5) like IOTA.

% There are sub-settings:
% \begin{itemize}
%     \item One caption setting: we only provide one caption for the algorithm.
%     \item Include ground truth setting: because some of the human tags are not in the captions, we manually include the tags into the candidate tags so that the model is able to predict. % rt: we no longer consider this.
% \end{itemize}


    % \rtcom{Need better layout.}\lior{hows this? can we resolve?} \rtcom{It is not clear which model the reconstructed caption from pillow is from.}}
    % \rtcom{I guess it's the best to trim the image, but there was a window there which makes the reconstructed caption really astonishingly correct. but I think it's fine.}\lior{I see. Ok, lets put a pin on this? not a priority now, rt: yes.}
    
    
%   \caption{Tag ranking (5-caption) with \tagcap models pre-trained different datasets. }


%  \lior{what are these nesting parentheses? can i remove it?}\rtcom{The (TF)IDF means that in this case TFIDF=IDF, I think it's confusing}\lior{lets challenge the reader and resolve ;)}

%   \rtcom{Do we need \tagcap+IOTA, in fact do we need \tagfeat+X in this table. for example tag2feat+tf, tag2feat+tfidf?}
% Tag ranking (5-caption). \tagc~and \tagf~are the abbreviation of \tagcap and \tagfeat respectively. Double lines separate single methods and ensembled methods.\rtcom{(proper?)  }
% LB: we need to descrobe the results. the entire caption is about notation..this might be the most important yet potentially confusing tables 
%  


==> signature.tex <==
\newgeometry{left=0in, right=0in, top=0in, bottom=0in}

\begin{figure}
 \centering 
 \includegraphics{figs/signatures.PDF}
\end{figure}


